On The Vulnerability of Anti-Malware Solutions to DNS Attacks

Anti-malware agents typically communicate with their remote services to share information about suspicious files. These remote services use their up-to-date information and global context (view) to help classify the files and instruct their agents to take a predetermined action (e.g., delete or quarantine). In this study, we provide a security analysis of a specific form of communication between anti-malware agents and their services, which takes place entirely over the insecure DNS protocol. These services, which we denote DNS anti-malware list (DNSAML) services, affect the classification of files scanned by anti-malware agents, therefore potentially putting their consumers at risk due to known integrity and confidentiality flaws of the DNS protocol. By analyzing a large-scale DNS traffic dataset made available to the authors by a well-known CDN provider, we identify anti-malware solutions that seem to make use of DNSAML services. We found that these solutions, deployed on almost three million machines worldwide, exchange hundreds of millions of DNS requests daily. These requests are carrying sensitive file scan information, oftentimes - as we demonstrate - without any additional safeguards to compensate for the insecurities of the DNS protocol. As a result, these anti-malware solutions that use DNSAML are made vulnerable to DNS attacks. For instance, an attacker capable of tampering with DNS queries, gains the ability to alter the classification of scanned files, without presence on the scanning machine. We showcase three attacks applicable to at least three anti-malware solutions that could result in the disclosure of sensitive information and improper behavior of the anti-malware agent, such as ignoring detected threats. Finally, we propose and review a set of countermeasures for anti-malware solution providers to prevent the attacks stemming from the use of DNSAML services.

==> sections/response-to-usenix-review.tex <==
\section{Response to USENIX Security '21 Fall}
We provide the review for a previous version of this manuscript by reviewers of the USENIX Security '21 Fall conference, and the authors' response.
The summary of changes is as follows:
\begin{enumerate}
    \item We modified the presentation of the problem and clarified that DNS anti-malware list (DNSAML) services are services with an architecture influenced by DNS domain block lists (DNSBLs) for anti-spam, used insecurely by anti-malware agents.
    \item The method for searching and identifying DNSAML services was reformulated and analyzed in every step for validation.
    Using the modified approach we were able to identify 55 services (compared to the previously identified seven services).
    \item The threat model is better motivated.
    Specifically, we clarify that today's man-in-the-middle attackers are very limited in their capabilities (due to the wide adoption of SSL). 
    This makes the capabilities of our threat model important and valuable to an attacker.
    \item The importance of the problem is better clarified using examples, screenshots, and demonstration videos on the most recent versions of the anti-malware agents evaluated.
    \item The attack validation methodology was rewritten for increased rigor and clarity.
    \item The set of proposed countermeasures is now compared using a set of nine criteria to describe the level of security, performance, compatibility, and flexibility.
    \item Before submitting the manuscript, it was reviewed by a native English speaker to improve the writing quality.
\end{enumerate}

The reviewers' concerns are presented based on the section of the revised manuscript that addresses the concerns, for easier verification.

\subsection{Introduction}
\noindent\textbf{Reviewer \#1:}
“The use of DNS for security lookup is nothing new. DNSBLs have been adopted by antispam tools since 2008”. \\

%“My main issue with this paper can be summarised in the response provided by McAfee in Appendix B. Yes, the use of DNS in reputation lookups used to be widely used, and yes the lack of encryption opens this to privacy constraints and, in some cases, may even led to potential for data tampering. But I feel that the spin given to this paper is wrong: there is nothing new in the use of DNS for this type of lookups. More specifically, DNSBL approaches were very very common in antispam filters since 2008. A variety of blacklists and data feeds used to be offered by various vendors (SURBL, DNSBL, ...), typically for free, on top of the DNS protocol. I don't find particularly surprising that these approaches exist, as they have been common practice for many years at the time in which a lot of the Internet traffic was not encrypted." \\

“In summary, I feel that the current spin of the paper (attempting to spin the discovery of a new vulnerability in cybersecurity applications) is a bit off the mark. There is something interesting in here, but the paper would need a mostly full rewrite in order to present the results as an analysis of the use of ``old" DNSBL techniques in the modern world.” \\

“- Modify the spin of the paper (the use of DNS for security lookups is not something unknown or newly discovered)” \\

\noindent \textbf{Response:}
%We thank the reviewer for his/her insightful comments. 
We agree with the reviewer that Domain Name System Block Lists (DNSBLs) began to be adopted by anti-spam tools over a decade ago, and therefore they are not a new tool for blocking spam. 
Furthermore, the use of DNSBLs to block spam is also properly documented~\cite{wiki:dnsbl} and has well-known criticism regarding its effectiveness in blocking spam and its legitimacy. \\
In this paper, we focus on \emph{the adoption of DNS security lookups by anti-malware sollutions}, which we denote DNS anti-malware list (DNSAML) services. 

In contrast to anti-spam DNSBLs, DNSAMLs aren’t well documented, and in our opinion, they have not been properly analyzed. 
The lack of a proper analysis and discussion is concerning given that the risks associated with tampering with decisions made by anti-malware solutions is arguably more important than anti-spam. 
To better set the stage for analyzing and discussing the impact of DNSAMLs, we accept the author’s proposal to modify the paper so as to frame DNSAMLs as a service with an architecture influenced by DNSBLs, rather than as a special use case of DNS data exchange. 
Accordingly, we modified Section~\ref{sec:intro} of the paper to support the re-framing as follows: \\

\color{red}
\hangindent=0.5cm
\textit{``The DNSAML service architecture is heavily inspired by that of Domain Name System Block Lists (DNSBLs)~\cite{wiki:dnsbl}, an architecture established to assist website administrators with blocking incoming connections from systems associated with spam.
The similar architecture provides DNSAML services with advantages like those of DNSBLs, such as ease-of-use and fast performance.
However, this architecture has disadvantages from the security perspective, because the DNS protocol is known to suffer from privacy and integrity flaws, such as a lack of source authentication and data encryption. 
These flaws enable a man-in-the-middle attacker to read, manipulate, and tamper with DNS packets without proper verification by the DNS protocol and its components~\cite{yan2020road,deccio2019dns}.
Therefore, anti-malware solutions that use DNSAML services without implementing additional safeguards may expose their solution and their consumers to various attacks that can result in information disclosure and affect decision-making.
For example, an attacker capable of manipulating DNS queries may respond on behalf of the DNSAML service and provide a false classification in order to incorrectly convince an anti-malware agent that a benign scanned file is malicious, or vice versa, causing the agent to delete benign files or maintain malicious files, respectively.''} \\
\color{black}

\subsection{DNS Anti-Malware List Services}
\noindent \textbf{Reviewer \#1}: 
“I do find that table 1 is much smaller than I would have expected: I would have expected you to find many more such examples.” \\

“A small improvement to the analysis performed in Section 3.2 is to convey a but more breakdown on the number of identified domains/organisations at the different stages of filtering.” \\

“- Include more details and insight on the analysis of the Akamai dataset (I'm quite surprised that so few DNS-based APIs are discovered)” \\

\noindent \textbf{Reviewer \#2}:
“More analysis and evaluations needed” \\

“The authors do not clearly describe how the ML analysis was made. Is it needed? Could you identify the same set of applications if you took the domains of all the security applications and checked queries to them in your dataset? Could you identify more security applications?" \\

\noindent \textbf{Response:}
%We address the concerns through the set of changes described below.
%First, we frame DNS anti-malware lists (DNSAMLs) as a special case of DNS security lookups, rather than as a special case of data exchange (see previous comment). 
Following the reviewers' comments, we updated our method of identifying DNSAMLs by first searching for \textit{any} active DNS security lookup services and then narrowing down the search to services operated for the benefit of anti-malware solutions. 
We also provide a more detailed analysis and evaluation.
In our search, we found 55 DNS security lookup services suspected to be DNSAML services, almost nine times more than appeared in the previous version of the manuscript.

To better support our analysis, we carefully read the documentation of these services to include only services that we could strongly argue to be related to anti-malware. 
We provide our documented evidence in Section 2.

The modified method relies on clearer actions that include:
\begin{enumerate}
    \item searching \emph{only} for domains that were categorized as security-related domains by Webroot;
    \item applying regular expressions to detect DNS queries that facilitate IP address and/or binary hashes commonly associated with DNSAML services, which arguably provides a clearer result than a machine learning model
\end{enumerate}

The evaluation provides a quantitative analysis for the number of domain names (DNS zones) identified in every step of the method, for improved verifiability of the results. 
In fact, the changes resulted in the identification of additional registered domains, as implied by the reviewer.

The set of changes appears in subsection~\ref{subsec:identify}: \\

\color{red}
\hangindent=0.5cm
\textit{
``The DNSAML services used by anti-malware solutions are expected to meet the following criteria:\\
\noindent \textbf{Active (C1)}: DNSAML services must process a high volume of DNS queries. \\
\noindent \textbf{Security-related (C2)}: The DNS zones (i.e., domain names) that are used to query the DNSAML services must be registered and owned by an anti-malware solution provider. \\
\noindent \textbf{Structured DNS communication (C3)}: DNS queries made to the service include IP address, binary hashes, and/or encrypted telemetries in various forms. }

\hangindent=0.5cm
\textit{Based on these criteria, we propose the following method to search for registered DNS zones suspected as DNSAML services:
\begin{tcolorbox}[left=0pt,breakable,title=\textit{DNSAML service search}]
\small
    \begin{enumerate}\leftmargin=1em
        \item \textbf{C1}: Collect $X_{C1}$: a distinct list of registered DNS zones that are queried at least $\theta$ times a day, on average, i.e., active domains
        \item \textbf{C2}: Collect $X_{C2}$: a list of domain names owned by security services, including anti-malware solution providers.
        %\item Create the set of suspected domains: $X_{C1 }=X_{C1} \cap X_{C2}$
        %\item Train a DNS tunneling classifier~\cite{nadler2019detection} on $X_{ACT}$: $F(\cdot)$
        \item \textbf{C3}: Collect $X_{C3}$: a list of registered DNS zones, whose DNS queries facilitate structured messages in $X_{C1} \cap X_{C2}$ as follows:
        \begin{enumerate}
            \item Create $S_{IP}$: the set of zones in $X_{C1} \cap X_{C2}$ for which at least 10\% of their DNS queries consist of a valid IPv4 address.
            \item Create $S_{HASH}$, the set of zones in $X_{C1} \cap X_{C2}$ for which at least 10\% of their DNS queries consist of a 32 character alphanumeric label.
            \item Create $S_{TUN}$ the set of zones in $X_{C1} \cap X_{C2}$ identified by a DNS tunneling classifier.
            \item $X_{C3} = S_{IP} \cup S_{HASH} \cup S_{TUN}$
        \end{enumerate}
        \item Return $X_{C1} \cap X_{C2} \cap X_{C3}$: a list of registered DNS zones satisfying C1, C2, and C3 and therefore suspected as DNSAML services.
    \end{enumerate}
\end{tcolorbox}
}

\hangindent=0.5cm
\textit{The set of active registered DNS zones $X_{C1}$ included 184,046 registered domain names that were queried at least $\theta=1000$ times per day, on average (i.e., $0.6\%$ of the registered zones in the dataset).
The set of security-related DNS zones $X_{C2}$ was established using Webroot BrightCloud, one of the world's largest web classification services.
Specifically, we extracted the ``Computer and Internet Security'' category, resulting in 220,426 domain names.
The intersection of active and security-related domains $X_{C1} \cap X_{C2}$ included $4,884$ registered DNS zones.
The set of DNS zones whose queries facilitate structured messages $X_{C3}$, consisting of less than $0.017\%$ of the registered DNS zones in the dataset, was extracted from $X_{C1} \cap X_{C2}$ for efficiency purposes.
The set $X_{C3}$ included 55 registered DNS zones, of which 43 consisted of IPv4 addresses ($S_{IP}$); ten consisted of 32 bit hashes ($S_{HASH}$), and 51 were identified by a DNS tunneling solution ($S_{TUN}$) proposed by Nadler et al.~\cite{nadler2019detection} to classify domain names related to DNS tunneling traffic.
The set of suspected DNSAML services $X_{C1} \cap X_{C2} \cap X_{C3}$ and their activity appears in Figure~\ref{fig:identifying} (in the manuscript), with their respective DNS queries per day (i.e., activity) and identification method, $S_{TUN}, S_{IP}, S_{HASH}$.
}
\color{black} \\

\textbf{Reviewer \#2:} ``Bullet 2: which remaining domains the organisations have registered?"\\

\noindent\textbf{Response:} The reviewer's concern refers to the previous method of identifying domains which relied on WHOIS information. 
The modified method makes use of the Webroot web categorization feed, and therefore, by definition, it provides the entire list of domains registered by security organizations that may be anti-malware solution providers.
The list is narrowed down based on the activity of DNS queries and the structure of DNS queries, therefore reducing the concern of excluding a relevant domain name due to its registration details. \\


\noindent\textbf{Reviewer \#2:} ``You use “scan” to refer to the query that the agent sends to the server. The “scan” in this case is confusing.” \\

%*** Asaf, Why not just saying that we changes the work scan to query? ***
\noindent\textbf{Response:} The use of the word ``scan" instead of "query" was indeed confusing; therefore, in the revised manuscript, the term ``scan" was replaced with "query." \\

%\noindent\textbf{Response:} We thank the reviewer for pointing out the confusion. 
%For better clarity, we made the following changes:
%\begin{enumerate}
%    \item Explain that the prevalence of anti-malware solutions use of DNSAML services must reflect the number of daily file scans for classification;
%    \item Estimate the number of daily file scans, by counting the number of DNS queries made to the DNSAML service, assuming that every DNS queries includes a file hash for scanning.
%\end{enumerate}

%The changes appear in subsection~\ref{subsec:prevalence} and %appear in red below: \\
%\color{red}
%\hangindent=0.5cm
%\textit{
%``The prevalence [of anti-malware solutions use of DNSAML services] is evaluated using three measures: the number of daily file scans for classification, number of communicating anti-malware agents, and number of origin countries from which the agents operate.''}\\

%\hangindent=0.5cm
%\textit{``The mean number of daily DNS queries to DNSAML services is 108 million, each assumed to include a binary file hash for classification.''}
%\color{black}


%\noindent \textbf{Reviewer \#2:} “In section 2.1 you refer to Authoritative name server extensions. Please explain what you mean."\\

%Section 3.2: the bulletpoint 1 starting with ``to select domains using multiple agents...." Not clear what the rationale for selection is and what you eliminated. \\

%\noindent \textbf{Response:} Both of the reviewer comments refer to parts that are no longer appear in revised manuscript.
%In particular, the term ``authoritative name servers'' was used to describe DNS forwarders, which are now coined using the latter term. 

\subsection{Threat Analysis}
\noindent \textbf{Reviewer \#2}: “The attacker is too strong, could do more significant attacks then just attack security applications.”\\

``You consider a strong attacker in this work. If you have a man-in-the-middle attacker, it can do more damage simply by poisoning the DNS cache and redirecting the queries to attackers’ servers hence subverting all the applications, not just security applications. The attacker can then inject or distribute malware without having to modify DNS responses to the security application. Can you please motivate and model your threat? Why is this significant? What additional threat does it introduce that an MitM attacker does not already have? Given such a strong attacker, does it gain more by launching your attacks?"\\

“Explain why the attacker model you use makes sense. Could an MitM attacker not do more significant attacks? Motivate why your threat gives attacker an additional capabilities.” \\

\noindent \textbf{Response:} Thank you for this important comment.
In the revised manuscript we better describe the motivation for our choice of the attacker model.
With the wide adoption of SSL for encrypting and signing web traffic, the capabilities of an MITM attacker have become fairly limited.
For example, a man-in-the-middle attacker may be able to redirect web traffic by spoofing DNS responses, however with SSL communication in place, exploiting a vulnerability within the browser or a social engineering attack is \textit{mandatory} in order for the attack \textit{to be successful without being detected}.
In our case, the plain-text DNS protocol allows an attacker to carry out the attacks \emph{secretly} and \textit{without the need for additional vulnerabilities}.
This makes the capabilities gained by exploiting the DNSAML technique extremely important and valuable for attackers. 

We revised the overview in Section~\ref{sec:threat_analysis} to provide these arguments as a motivation for our threat model: \\

\color{red}
\hangindent=0.5cm
\textit{``Based on a previous threat analysis of the DNS~\cite{atkins2004threat} and recently published DNS cache poisoning attacks \cite{herzberg2012security,man2020dns,klein2020cross}, we consider three type of attackers that can acquire the abovementioned capabilities: a man-in-the-middle attacker, an off-path attacker with IP spoofing capability that controls an adjacent machine, and an off-path attacker without any additional capabilities.}

\hangindent=0.5cm
\textit{Today, with the wide adoption of SSL for encrypting and signing web traffic, the capabilities of the different attackers are very limited.
A man-in-the-middle attacker may be able to redirect web traffic by spoofing DNS responses.
However, with SSL encryption in place, the attacker must perform a social engineering attack or exploit a vulnerability within the browser in order for the attack to be successful and go undetected.
In our case, the plain-text DNS protocol allows an attacker to carry out the attacks described below \emph{secretly} and without the need to exploit additional vulnerabilities.
This makes the above-mentioned capabilities extremely important and valuable to attackers."}
\color{black}
\\

\noindent \textbf{Reviewer \#1:} “From a threat model perspective, there is a significant difference in using the attack to turn a malicious item to benign vs doing the opposite``\\

“I'm not fully convinced that the problem is as serious as it is being presented”\\

\noindent \textbf{Response:} The additional capabilities that the attacker acquires are: (1) the ability to perform host-based manipulation without a host-based presence; (2) the ability to perform the manipulation silently, without any side-effect/alert to the client; and (3) the ability to “target” specific messages (or malware scans).
In the case of secure communication  (i.e., confidentiality and integrity), a man-in-the-middle attack can only disable all of the communication with a remote anti-malware service, which is very noisy and can be easily detected by the user.


\noindent \textbf{Reviewer \#1:} “Please provide more information on the “Sensitive information” that “can be collected by the attacker for reconnaissance purposes, in order to assess the security posture of the target machine, thus resulting in the disclosure of sensitive information”. Also please explain what is contained in the security posture.” \\

\noindent \textbf{Response:} We include the information requested by the reviewer in Section~\ref{sec:threat_analysis}:\\

\color{red}
\hangindent=0.5cm
\textit{``The queries made by anti-malware agents to DNSAML services to agents provide information regarding scanned files.
Accordingly, an attacker with a DNS eavesdropping capability can intercept the queries made an agent to its DNSAML service to gain information about scanned files.
With this information, a threat actor spreading malware can (a) determine whether a specific malware was successfully delivered to a victim endpoint without being detected; (b) learn which known malware go undetected by a DNSAML service and deliver them to the victim; and (c) assess the security posture of an organization based on the number of file scans, their file information and their responses that indicate the rate of malicious downloaded files by that organization.''}
\color{black}
\\
\subsection{Attacks On DNSAML Services}
\noindent \textbf{Reviewer \#1:} “- **Silencing attack**. I am not convinced that this scenario is realistic. All the APIs involved in the analysis are simple blacklists of IPs or hashes, a very low sophistication detection tool that is not really meant to provide any real protection against advanced threats. An attacker attempting to bypass an IP blacklist can very cheaply obtain a clean IP at very low cost (VPNs, TOR, botnets) without the need to carry out a much more costly Mitm attack on the DNS protocol. An attacker attempting to bypass a hash reputation API can even more cheaply modify the hash of its trojan to escape detection.” \\

\noindent \textbf{Response:} We respectfully disagree with the reviewer's comment. Our experimental setup, shown in Section~\ref{sec:in-depth}, shows that these attacks were successfully applied to recent versions of anti-malware agents by well-knwon vendors, such as McAfee Endpoint Security Threat Prevention (ESTP) version 10.6.1.1386.8 and Tenable's Nessus Professional Version 8 (8.11.1).
In both cases, we managed to show that an attacker with DNS tampering capability is able to manipulate these agents to completely ignore malware in scan reports and accordingly allow their execution on a victim machine.\\

Furthermore, to demonstrate that this scenario is realistic, we include videos and screenshots.
The screenshot (see Figure~\ref{fig:mcafee-silencing-screenshot}) shows the differences between the scanning of a malicious file without attack and with the silencing attack on the McAfee ESTP agent.
Without the attack, the Artemis Trojan is successfully detected by the agent, that takes the action of deleting the Trojan file.
In contrast, when the silencing attack is carried, the attacker spoofs the DNS responses made by McAfee's GTI DNSAML service to the agent, which results in an empty scan report. 
As a result, the malicious Artemis Trojan, is ignored by the agent and is allowed to be executed on the victim machine.\\

\noindent \textbf{Reviewer \#1:} “- **False alert attack**. Among all the attack schemes presented, this is the most convincing one with respect to the threat model. An advanced attacker able to put himself in a Mitm position could potentially abuse the described DNS channels to block and remove arbitrary files from the targeted systems with potentially catastrophic consequences. However, the only tool analysed in the paper where this attack would be possible is McAfee GTI, but this service implements protections against this attack by including a cryptographic exchange to verify the hit. All the other tools do not have capability to action the false positives other than generating an alert. This would be an annoyance for an operator, but a relatively small gain compared to the cost of implementing the attack…”\\

\noindent \textbf{Response:} We respectfully disagree with the view of the reviewer by which alert fatigue is a small annoyance. By a recent McAfee report~\footnote{https://www.mcafee.com/blogs/enterprise/cloud-security/alert-fatigue-31-9-of-it-security-professionals-ignore-alerts/}, among IT security professionals, 31.9\% report that they ignore alerts because so many are false positives. This statement arguably convinces that alert fatigue either reduces the security effectiveness of the victim, or conversely, forces the victim to invest in more IT security professionals to handle false alerts. Both of these cases imply that alert fatigue must not be undervalued. \\

Additionally, the false alerts attack inflicts damage not only to the victim; it also damages the brand of the anti-malware solution provider. The attack causes the anti-malware solution to present the victim with inaccurate reports, which in turn may lead to lack of trust by the solution consumers. We revised Section~\ref{sec:threat_analysis} to properly reflect that: \\

\color{red}
\hangindent=0.5cm
\textit{``The responses made by DNSAML services to agents indicate whether a scanned file is malicious. 
Accordingly, an attacker with limited or complete DNS tampering capability can spoof the DNSAML response cause an agent to incorrectly classify a benign file as malicious. 
Such an attack will result in alert fatigue, and potential sanctions against a benign file.
Furthermore, the inaccurate reports resulted by this attack, may damage the brand of the anti-malware solution provider, and the trust of its consumers."}
\color{black}
\\

\noindent \textbf{Reviewer \#1:} ``I may find surprising if such techniques are still being used by the latest version of a product sold in 2020. But even in that case, the paper fails to properly analyse the impact and the role of these DNS channels in the involve product and its threat model.” \\

\noindent \textbf{Response:}
The experimental setup described in Subsection~\ref{subsec:experimental_setup} provides details about the anti-malware agents used for the evaluation; in this subsection, we emphasize that \emph{all} agents were released and available in 2020: \\

\color{red}
\hangindent=0.5cm
\textit{``\noindent \textbf{Victim Setup:} To simulate the victim, we set up a virtual machine (VM) with the recent Windows 10 operating system using a VMware workstation.
The VM is connected to the Internet to allow the installed agent to query its DNSAML service.
In each experiment, we install the most recent version of the inspected malware agent, namely:
\begin{enumerate}
    \item McAfee Endpoint Security Threat Prevention (ESTP) version 10.6.1.1386.8, or
    \item Nessus Professional Version 8 (8.11.1), or
    \item python-tools-cymru~\cite{python-cymru-tools}
\end{enumerate}"}
\color{black}
\\

Furthermore, the response to the responsible disclosure by the anti-malware solution providers confirms that at the time of disclosure, their recent versions did indeed support the insecure use of DNSAML services  (see Appendix~\ref{sec:responsible_disclosure}).\\
In particular, McAfee confirmed that at the time of the responsible disclosure, they were working actively on migrating the use of GTI-DNS to GTI-REST, one of the solutions proposed in the manuscript. \\
%\color{red}
%The latest evolution of our GTI service is GTI-REST. 
%This runs only over TLS 1.2 and does not support unauthenticated clients. Our GTI-REST POPs receive an A rating from SSL Labs. 
%Our effort to move the remaining core products from GTI-DNS to this new GTI-REST service was already underway when we received the report.''
%\color{black}
%\\

\noindent \textbf{Reviewer \#1:} “I think that this part of the paper could have benefited from a bit more structure and rigor (e.g. in 5.1.2 you mention ``Through extensive analysis", that's quite vague: what type of analysis? what methodology was employed?) it is still a laudable attempt.” \\

“More formally describe the testing methodology against the various products analysed in the paper” \\

\noindent \textbf{Response:} We agree with the reviewer's comment. 
Accordingly, we dedicated an entire subsection to the attack validation methodology (see Subsection~\ref{subsec:validation}): \\

\color{red}
\hangindent=0.5cm
\textit{``In order to validate the feasibility of the three attacks, we construct a setup of benign and malicious files, and the set of DNS responses returned by the inspected DNSAML service.
We use the notations described below:}

\begin{tcolorbox}[left=0pt,title=\textit{Setup}]
    \small
    \begin{enumerate}\leftmargin=1em
        \item $F_{B}$: a set of benign files
        \item $F_{M}$: a set of malicious files
        \item $R_{O}$: the set of DNS responses returned from the DNSAML service through observations
        \item $A_{B}$: the set of predetermined actions for benign files: \emph{ignore}
        \item $A_{M}$: the set of predetermined actions for malicious files: \emph{delete, quarantine or report}
    \end{enumerate}
\end{tcolorbox}

\hangindent=0.5cm
\textit{To validate the information disclosure attack (\textit{\textbf{ATT-ID}}), we set up two different endpoints and install the anti-malware agent associated with the DNSAML.
Then, we deploy the same file onto both endpoints, and observe the outgoing DNS queries to the DNSAML service.
We assert that the information disclosure attack is feasible for a specific DNSAML service if and only if the outgoing DNS queries made from both endpoints match exactly i.e., the reported signatures are independent of the endpoint, and depends only on the scanned file.
This assertion implies that an attacker capable of DNS eavesdropping that seeks to learn whether a victim downloaded a \emph{specific} file, can generate the reported signature using its own setup, and then match that signatures upon DNS eavesdropping.
The validation process of the information disclosure attack is described below:}

\begin{tcolorbox}[left=0pt,title=\textit{Information Disclosure Attack Validation}]
\small
    \begin{enumerate}\leftmargin=1em
        \item Let $e1, e2$ be two different endpoints with the same anti-malware agent installation.
        \item For every file $f^{i}$ in $F_{B} \cup F_{M}$:
        \begin{enumerate}
            \item Deploy the $f^{i}$ onto $e1$ and record the first DNS query made to the DNSAML service: $q(f^{i}, e1)$
            \item Deploy the $f^{i}$ onto $e2$ and record the first DNS query made to the DNSAML service: $q(f^{i}, e2)$
            \item If $q(f^{i}, e2) \neq q(f^{i}, e2)$, return False
        \end{enumerate}
        \item Return True
    \end{enumerate}
\end{tcolorbox}

\hangindent=0.5cm
\textit{To validate the false alerts attack (\textit{\textbf{ATT-FA}}), we deploy benign files onto an endpoint protected by the anti-malware agent associated with the inspected DNSAML service.
For every deployed file, we record the DNS response returned from the DNSAML, and agent \emph{behavior} towards the file i.e., delete, quarantine, report or ignore.
After recording this information, we redeploy each file, while subverting the DNS response returned by the DNSAML service, and check whether the behavior changed.
Specifically, the set of subverted responses is extracted from the set of responses made by the DNSAML on our dataset, therefore limiting the search.
We claim that an attack capable of DNS tampering, can launch the false alerts attack if and only if for every file, at least one subverted response results in changing the agent behavior from ignore to delete, quarantine or report.
The validation process of the false alert attack is described below:}

\begin{tcolorbox}[left=0pt,title=\textit{False Alerts Attack Validation}]
\small
    \begin{enumerate}\leftmargin=1em
        \item Let $V=\emptyset$ be the set of benign files on which the attacker resulted in a false alert
        \item For every file $f^{i}_{B}$ in $F_{B}$:
        \begin{enumerate}
            \item Deploy the $f^{i}_{B}$ onto the endpoint
            \item Record the DNSAML service response $r(f^{i}_{B})$
            \item Record the agent's action for the file: $a(f^{i}_{B}, r(f^{i}_{B}))$
            \item Verify $a(f^{i}_{B}, r(f^{i}_{B})) \in A_{B}$; otherwise, return False.
            \item For every response $r_{j}$ in $R_{O}$:
            \begin{enumerate}
                \item Deploy the $f^{i}_{B}$ onto the endpoint
                \item Subvert the DNS response $r(f^{i}_{B})$ to $r_{j}$
                \item Record the action : $a(f^{i}_{B}, r_{j})$
                \item If $a(f^{i}_{B}, r_{j}) \in A_{M}$, then $V = V \cup \{f^{i}_{B}\}$
            \end{enumerate}
        \end{enumerate}
        \item Return True if $V = F_{B}$
    \end{enumerate}
\end{tcolorbox}

\hangindent=0.5cm
\textit{To validate the silencing attack (\textit{\textbf{ATT-S}}), we deploy malicious files onto an endpoint protected by the anti-malware agent associated with the inspected DNSAML service.
For every deployed file, we record the DNS response returned from the DNSAML, and agent \emph{behavior} towards the file i.e., delete, quarantine, report or ignore.
After recording this information, we redeploy each file, while subverting the DNS response returned by the DNSAML service, and check whether the behavior changed.
Specifically, the set of subverted responses is extracted from the set of responses made by the DNSAML on our dataset, therefore limiting the search.
We claim that an attack capable of DNS tampering can launch the silencing attack if and only if for every file, at least one response subversion results in changing the agent behavior from delete, quarantine or report to ignore.}

\begin{tcolorbox}[left=0pt,title=\textit{Silencing Attack Validation}]
    \small
    \begin{enumerate}\leftmargin=1em
        \item Let $V=\emptyset$ be the set of malicious files which the attacker made the agent ignore
        \item For every file $f^{i}_{M}$ in $F_{M}$:
        \begin{enumerate}
            \item Deploy the $f^{i}_{M}$ onto the endpoint
            \item Record the DNSAML service response $r(f^{i}_{M})$
            \item Record the agent's action for the file: $a(f^{i}_{M}, r(f^{i}_{M}))$
            \item Verify $a(f^{i}_{M}, r(f^{i}_{M})) \in A_{M}$. Otherwise, return False.
            \item For every response $r_{j}$ in $R_{O}$:
            \begin{enumerate}
                \item Deploy the $f^{i}_{M}$ onto the endpoint
                \item Subvert the DNS response $r(f^{i}_{M})$ to $r_{j}$
                \item Record the action : $a(f^{i}_{M}, r_{j})$
                \item If $a(f^{i}_{M}, r_{j}) \in A_{B}$, then $V = V \cup \{f^{i}_{M}\}$
            \end{enumerate}
        \end{enumerate}
        \item Return True if $V = F_{M}$
    \end{enumerate}
\end{tcolorbox}
\color{black}

\noindent\textbf{Reviewer: \#2:} “The scan report that is returned in Section 5.1.2 – is it returned over DNS? You describe the report which is over HTTP. Is the eavesdropping attacker sees the plaintext access over HTTP? Or is this over DNS?" \\

\noindent \textbf{Response:} The DNS eavesdropping attacker considered in manuscript can only intercept plain-text DNS traffic; the attacker \emph{cannot} intercept any HTTP or HTTPS traffic.
However, using the infromation disclosure attack, an DNS eavesdropping attacker can learns the hashes of scanned files based on the victim's outgoing DNS queries.
The scan report is returned over HTTP. However, the URL of the scan report is: ``\url{http://malwaredb[.]nessus[.]org/malware/<file_hash>}''.
Accordingly, by browsing the above-mentioned URL and appending the hash, the attacker can browse the report provided by Tenable regarding the file.
We revised section~\ref{subsec:in-depth}) to clarify that:\\

\color{red}
\hangindent=0.5cm
\textit{``Every malware scan results in a scan report.
Within the scan report, every file that is identified as malicious is associated with the number of security engines by which it was scanned and the number of engines that classified the file as malicious. In some cases, the report also indicates which particular engines considered the file as malicious.
In addition, the scan report assigns each malicious file with a report that users can browse by visiting a URL.
The URL is http://malwaredb[.]nessus[.]org/malware/ followed by the file hash.
The report contains the MD5 hash of the scanned file, as well as a detailed description of the malware, thus allowing an eavesdropping attacker to obtain a standard hash that can be matched against other services."
}
\color{black} 

\noindent \textbf{Reviewer: \#2:} ``It is a pity that the details on the reversible function are missing from the paper – this makes it difficult to be able to judge it or understand this result. Same with a function in Section 5.1.4" \\

\noindent \textbf{Response:} We included the details on the reversible function in Sub-subsection~\ref{subsubsec:mhr}:

\color{red}
\hangindent=0.5cm
\textit{``Furthermore, we found consistencies between labels appearing in the malicious responses and attributes appearing within the scan report.
For instance: The third and fourth octet represent 16 ordered flags, each for a specific engine that classified the file as malicious.
Based on that, we were able to reconstruct a function that associates the report results to the IP address response, and vice versa, thus allowing an eavesdropping attacker to learn the report results simply by applying the function to the IP addresses contained in the responses.
The reversible function that translates the IP address contained in the response to a scan report is redacted from this paper for the sake of responsible disclosure.}

\hangindent=0.5cm
\textit{The function that maps IP addresses contained in the responses to the report results is defined as follows:
\begin{enumerate}
    \item The first three (MSB) bits (left-most) of the first octet  are ignored.
    \item The remaining five bits of the first octet form a binary representation of the total number of engines that scanned the file. 
    \item The last five (LSB) bits of the second octet form a binary representation of the number of engines that classified the file as malicious.
    \item The third and fourth octet represent 16 ordered flags, each for a specific engine that classified the file as malicious.
\end{enumerate}}
\color{black} 

\noindent\textbf{Reviewer: \#2:} “The attacks, in Section 5.3.1, how does a dictionary look for each application? What does it contain?” \\

\noindent\textbf{Response:} We revised the manuscript to better explain that the dictionary includes a set of malicious file hash strings, as specified by the outgoing DNS queries made by the agent to the DNSAML service.
We will demonstrate the latter using an example.
A DNS eavesdropping attacker learns that the victim machine has Tenable's Nessus Professional agent installed.
The attacker attempted to infect the victim machine with a specific malware and now seeks to learn whether the victim successfully downloaded the file.
Accordingly, the attacker sets up a machine with the same agent and deploys its malware on the machine.
After issuing a malware scan, the Nessus agent on the attacker setup issues the following DNS query:
\[
257afb596ee35de6695adc620e24f362.l2.nessus.org.
\]
Based on that query, the attacker constructs a dictionary set that includes a single string:
\[
    \{ ``257afb596ee35de6695adc620e24f362'' \}
\]
After the setup phase, the attacker starts intercepting the victim's DNS traffic and attempts to match the file hash in the dictionary. 
If successful, the attacker concludes that if the DNS query was indeed made by the Nessus agent, which is most likely; then the victim successfully downloads the attacker's malware.

We revised the description of the attack in Subsection~\ref{subsec:attacks} for improved readability: \\

\color{red}
\hangindent=0.5cm
\textit{
\textbf{Information Disclosure Attack (ATT-ID):} This attack realizes the information disclosure threat described in Section~\ref{sec:threat_analysis}.
In this attack, an attacker with a DNS eavesdropping capability seeks to learn whether a \emph{specific} set of malware is downloaded from a machine owned by the victim.
The attack includes the following steps:
\begin{enumerate}
    \item The attacker learns which anti-malware agent is installed on the victim machine by intercepting the victim's outgoing DNS queries, and matching the DNS zones to DNSAML services described in Section~\ref{sec:usingdns}.
    \item The attacker sets up a machine with an anti-malware agent similar to that installed on the victim machine 
    \item The attacker deploys a set of malware onto its machine and inspects the outgoing DNS traffic made from the agent to the DNSAML service.
    \item The attacker constructs a dictionary of file hashes that appear in the outgoing DNS traffic to the DNSAML service (step 0).
    \item The victim machine downloads a file (step 1)
    \item The attacker intercepts the victim's DNS outgoing traffic (step 2), and matches every DNS query made to the DNSAML service, with the set of hashes within the dictionary (step 3).
    \item Every successful match, indicates that a DNS query was made, most likely by the victim's installed agent, therefore indicating the victim's machine contains one of the malware within the set.
\end{enumerate}
The attack scenario is illustrated in Figure~\ref{fig:info_disc}).}
\color{black} \\

\noindent\textbf{Reviewer: \#2:} “Provide technical details about the analysis and evaluation (see more questions in comments for authors).” \\

\noindent\textbf{Response:} 
Following the revision of the attack validation methodology, we also provide further details on the experimental setup, to accurately describe the technical details of our analysis.
The experimental setup appears in Subsection~\ref{subsec:experimental_setup} as follows: \\

\color{red}
\hangindent=0.5cm
\textit{
\noindent \textbf{Attacker Setup:} To simulate the attacker, we set up a virtual machine with Kali Linux. 
The attacker machine resides as a MITM between the victim machine and the Internet. 
The DNS interception and spoofing were conducted with the Ettercap tool (for both ARP poisoning and DNS spoofing), running on a physical Linux machine, connected to the same LAN as the victim.
}
\\
\hangindent=0.5cm
\textit{
\noindent \textbf{Victim Setup:} To simulate the victim, we set up a virtual machine (VM) with the recent Windows 10 operating system using a VMware workstation.
The VM is connected to the Internet to allow the installed agent to query its DNSAML service.
In each experiment, we install the most recent version of the inspected malware agent, namely:
\begin{enumerate}
    \item McAfee Endpoint Security Threat Prevention (ESTP) version 10.6.1.1386.8, 
    \item Nessus Professional Version 8 (8.11.1), or
    \item python-tools-cymru~\cite{python-cymru-tools}
\end{enumerate}}

\hangindent=0.5cm
\textit{
\noindent \textbf{The Benign and Malicious Files:}
The set of benign files includes 10 new Microsoft Office documents of various formats that we created and could confirm to be benign.
To construct the set of malicious files, we had to obtain files that the inspected anti-malware solution ``believes'' to be malicious.
This requirement was critical to guarantee that the DNSAML service's response instructs the agent to perform the malicious action. }

\hangindent=0.5cm
\textit{
In the case of Tenable's MalwareDB, we extracted MD5 file hashes that we observed within the DNS traffic whose DNS response was extremely rare (i.e., less than 0.1\% of all DNS queries).
For instance, the query b48eb0932dfb629ce70d7142ceb74a13.l2.nessus.org. was observed only once within the 30-day period, and therefore we extracted the file hash ``b48eb0932dfb629ce70d7142ceb74a13.''
In turn, we used the VirusTotal service to download the malicious files based on its MD5 file hash.
Overall, we used seven files that we were confident the Nessus agent would classify as malicious. \\
In the case of McAfee GTI, we faced greater difficulty, since the file hash used was not MD5 or SHA1, which are the known standards for malicious file hashes.
Accordingly, we were unable to download malicious files directly from VirusTotal.
Instead, we carefully modified two malicious binaries to form 10 files which we manually confirmed to be new and were classified as malicious by the DNSAML service. \\
In the case of Team Cymru, we used the example of malicious file hash demonstrated in their guidelines~\cite{cymru_mhr}.}
   \\
 \\
\hangindent=0.5cm
\textit{
In the case of Team Cymru's MHR, we used the example of malicious file hashes demonstrated in their guidelines~\cite{cymru_mhr}."}
\color{black}

\subsection{Proposed Countermeasures}
\noindent\textbf{Reviewer \#1:} “In various parts of the paper you seem to suggest that it is common to find network policies where the DNS protocol is allowed, but HTTP/HTTPS is not. 
I would love to see some proof of this assumption (the vast majority of update protocols for any kind of software even on servers uses HTTP/HTTPS).” \\

\noindent\textbf{Response:} The reviewer points out a valid concern --- it is unclear that the anti-malware solutions are ever \emph{forced} to use the DNS protocol to exchange information regarding scanned files.
Accordingly, we re-framed the considerations for anti-malware solution providers to select the use of DNSAML services to a more relaxed consideration: backward compatibility.
The consideration of compatibility is described in Sub-subsection~\ref{subsubsec:compatibility} as follows: \\

\color{red}
\hangindent=0.5cm
\textit{
\textbf{Compatibility.} The criteria in this category examine the difficulty of implementing the countermeasure and the effort required by consumers to integrate it. The motivation for including this criterion stems from the fact that anti-malware solutions are sometimes installed on servers with a strict network policy, such as email gateways~\cite{symantec_brightmail} or secure web gateway (SWG) proxies. 
In such scenarios, consumers that anticipate malware tend to reduce the attack surface on the server by allowing a limited set of Internet protocols, for instance, allowing outbound DNS but blocking outbound HTTP/S. Given the use of DNSAML services, we know that DNS is allowed by definition. 
Allowing encrypted DNS will therefore require some effort, and other protocols may be more difficult or infeasible under strict network policies.}
\color{black}.
\\

We argue that while DNSAML services are not a necessity, anti-malware providers that currently use it still are faced with the concern of costs associated with interfering with existing compatibility, as explained above.
Accordingly, we include the compatibility category as one of four categories as a countermeasure alternative for DNSAML services.\\

\noindent\textbf{Reviewer \#1:} “In Section 6.1 you propose as solution to prefer HTTPS and fallback on DNS in case of communication issues. I don't believe this would address your threat model: if an attacker is in a Mitm position, he can very equally inject RST packets to prevent HTTPS communication to succeed.” \\

\noindent \textbf{Response:} The reviewer is correct. 
Furthermore, because we now argue that the DNS protocol is \emph{not} a necessity for exchanging scanned file information (see previous comment), we no longer support the proposed solution that the reviewer refers to.
Rather, we focus on four countermeasures (see Section~\ref{sec:countermeasures}), without using any fallback to plain-text DNS. \\

\noindent \textbf{Reviewer \#1:}  “Similarly in Section 6.1, you investigate various approaches to use secure versions of DNS to perform the lookups. Why misusing the DNS protocol to do something it is not designed for instead of using Restful APIs (as McAfee mentions in its response)?” \\

\noindent \textbf{Response:} Following the reviewer's comment, we revised the solution section to compare four proposed countermeasures (including REST APIs) on four categories of criteria.
Our review finds that REST APIs are in a secure countermeasure; they are also flexible, given their ability to support future extensions, because they are not limited to 255 characters, like the DNS protocol.
However, RESTful APIs have two disadvantages compared to the other countermeasures when considered as alternatives to existing DNSAML services, namely their performance and compatibility.
From the performance perspective, existing queries over the DNS protocol to DNSAML services outperform RESTful APIs, because they have native support for caching on DNS resolvers, and they are sent over the UDP transport layer therefore incurring the lowest response time overhead of all of the examined countermeasures.
From a compatibility perspective, both anti-malware solution providers and consumers must adapt their infrastructure and network policies to support a transition to RESTful APIs, an effort that is significantly greater than that associated with DoH or DoT.
We discuss these considerations regarding the RESTful APIs in Subsection~\ref{subsec:countermeasures}: \\

\color{red}
\hangindent=0.5cm
\textit{\noindent\textbf{``REST APIs}~\cite{wiki:restapi} is a standard for a software architecture for interactive Web applications.
Compared to previous solutions, this solution proposes to deprecate the DNS protocol for exchanging signatures, and make use of HTTPS.
The main upside of REST APIs are its security and flexibility, since compared to DNS, it allows larger messages (i.e., up to 2MB with GET requests).
In contrast, it has the worst performance and compatibility issues compared to the other solutions, because providers are required to change their infrastructure to support HTTPS, and consumers are required to permit HTTPS."}
\color{black}
\\

\noindent \textbf{Reviewer \#2:} “The countermeasures should also address shortcomings of the proposals, such as attacks against DNS encryption proposals.”\\

“In the proposed countermeasures, the authors propose using DNS encryption to ensure privacy. In the recent years a number of attacks against such solutions were demonstrated. Your should list those and explain how these impact your recommendation to use DNS encryption solutions. Would the techniques proposed in prior work for inferring the encrypted input enable your attacks despite encryption?”
“Add reference to attacks against DNS encryption proposals.” \\

\noindent \textbf{Response:} We updated the manuscript to discuss the security limitations of the proposed countermeasures, particularly encrypted DNS protocols.
The revised text appears in Subsection~\ref{subsec:countermeasures}: \\

\color{red}
\hangindent=0.5cm
\textit{
\noindent\textbf{DNS over TLS (DoT)}~\cite{zhu2015connection} is privacy-preserving protocol based on a combination of the TCP stack and TLS that is used to improve DNS security and reliability. 
In DoT, DNS data is encrypted, which in turn reduces the impact of various DNS attacks (e.g., DNS hijacking) by establishing mutual connections. 
DNS based on TLS is designed to provide greater privacy, support large payloads, and mitigate hijacking and reflection distributed denial-of-service attacks more effectively than existing UDP protocols.
DoT provides a security countermeasure against all of the mentioned threats, by design.
The main security limitation of this countermeasure is privacy leakage~\cite{houser2019investigation, bushart2020padding}, allowing an MITM attacker to learn whether a user visits a specific set of domains, which is arguably a lesser concern than learning which \emph{exact} files are being scanned by a machine, but is still a concern.
From a performance perspective, the use of the TCP transport layer result in reduced performance compared to the DNS protocol over the UDP transport layer.
However, caching is still supported, similarly to DNS without TLS.
To support DoT in anti-malware solutions, consumers need to allow the DoT port (853), and solution providers must replace the DNS resolver with a DoT resolver.}

\hangindent=0.5cm
\textit{
\noindent\textbf{DNS-over-HTTPS (DOH)}~\cite{rfc8484} is a standard web protocol for sending DNS traffic over the privacy-preserving HTTPS. 
DoH provides a security countermeasure against all of the attacks mentioned.
Its main security limitation is its susceptibility to downgrade attacks~\cite{huang2020comprehensive} that force an client (e.g., agent) to fall back to plain-text DNS.
From a performance perspective, the use of HTTP incurs more overhead than to plain-text DNS, and caching is only supported at the recursive DNS server level and not within internal servers, as in the case of plain-text DNS.
To support DoH in anti-malware solutions, consumers need to allow HTTPS traffic, and solution providers must replace the DNS resolver with a DoH resolver.}
\color{black}
\\

These limitations are also included in the summary of proposed countermeasures (see the security column in Table~\ref{tab:countermeasures}). \\

\subsection{General concerns (Writing quality and minor comments)}
\noindent \textbf{Reviewer \#2:} “The paper is poorly written and the text is difficult to parse. For instance, “The results over time are presented over time in Figure 2, and their describing statistics appear in Table 2”.
“In our experiments which involved several scans, we witnessed file scans for which two specific IPv4 addresses were provide in response, resulting in a situation in which the file was not designated as malicious in the scan report;”. \\

\noindent \textbf{Response:} Before submitting the manuscript, it was reviewed by a native English speaker to improve the writing quality.

\noindent\textbf{Reviewer \#1:} ``The HTTPS protocol is typically spelled HTTPS and not HTTPS'' \\

\noindent \textbf{Response:} We replaced all instances of the term ``HTTPs'' with ``HTTPS.'' \\


==> sections/solutions-short.tex <==
\section{\label{sec:countermeasures}Proposed Countermeasures} 
In this section, we review a set of countermeasures to prevent attacks stemming from the use of DNSAML services (see Section~\ref{sec:in-depth}).
The set of countermeasures include: application-level signing, DNS-over-HTTPS~\cite{rfc8484}, DNS-over-TLS~\cite{zhu2015connection}, and REST APIs, which are further described on Appendix~\ref{subsec:countermeasures}.
The countermeasures are assessed by categories of assessment criteria we define: security, performance, compatibility, and flexibility (see full definition in Appendix~\ref{subsec:countermeasures_methodology}).
The following symbols (\CIRCLE,\LEFTcircle,\Circle) are used to indicate whether a criterion is fully satisfied, partially satisfied, or not satisfied by a countermeasure.

The summary of the countermeasures is presented in Table~\ref{tab:countermeasures}.
Our interpretation of the summary is as that (1) application-layer signing strongly favors performance and consumer compatibility over security, provider compatibility, and flexibility; (2) DoH and DoT provide a reasonable balance between performance and compatibility; and (3) REST APIs were found to be the least compatible of the countermeasures, but they provide ideal security and flexibility.
In their response to our responsible disclosure, McAfee indicated that it intends to enable REST APIs as their sole countermeasure, while Team Cymru plans on employing both plain-text DNS and REST APIs to assure backward compatibility.

\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
                  & \multicolumn{4}{c|}{Security}       & \multicolumn{2}{c|}{Performance}     & \multicolumn{2}{c|}{Compatibility} & Flexibility        \\ \hline
Countermeasure & \textbf{ATT-FA} & \textbf{ATT-FA} & \textbf{ATT-S} & \begin{tabular}[c]{@{}l@{}}Known \\ Limitations\end{tabular} & \begin{tabular}[c]{@{}l@{}}Response Time \\ Overhead \end{tabular} & Caching & \begin{tabular}[c]{@{}l@{}}Negligible \\ Infra. Changes\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Negligible \\ Consumer Effort\end{tabular}    & \begin{tabular}[c]{@{}l@{}}Character \\ Limitation\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}DNSAML services \\ without implementing \\ additional safeguards\end{tabular}                  & \Circle  & \Circle  & \Circle  &  & \Circle & \CIRCLE & \CIRCLE  & \CIRCLE       & \Circle  \\ \hline
Application-layer signing & \Circle & \CIRCLE & \CIRCLE &  & \LEFTcircle & \CIRCLE & \Circle  & \CIRCLE       & \Circle  \\ \hline
DoT~\cite{zhu2015connection} & \CIRCLE & \CIRCLE & \CIRCLE & ~\cite{houser2019investigation, bushart2020padding} & \LEFTcircle & \CIRCLE & \LEFTcircle & \LEFTcircle & \Circle  \\ \hline
DoH~\cite{rfc8484}                          & \CIRCLE & \CIRCLE & \CIRCLE & \cite{huang2020comprehensive} & \LEFTcircle & \Circle  & \LEFTcircle & \Circle        & \Circle  \\ \hline
REST APIs~\cite{wiki:restapi}                    & \CIRCLE & \CIRCLE & \CIRCLE &  & \Circle & \Circle  & \Circle & \Circle        & \CIRCLE \\ \hline
\Xhline{3\arrayrulewidth}
\multicolumn{10}{l}{Security -  \textbf{ATT-ID}: Information Disclosure attack , \textbf{ATT-FA}: False Alert attack, \textbf{ATT-S}: Silencing attack.} \\
\multicolumn{10}{l}{Fully satisfies (\CIRCLE), partially satisfies (\LEFTcircle), does not satisfy (\Circle).} \\
\end{tabular}%
}
\caption{Summary of proposed countermeasures to limit the consequences of attacks stemming from the insecure use of DNSAML services on anti-malware solutions and their consumers.}\label{tab:countermeasures}
\end{table*}


